Automatic Differentiation of Programs with Discrete Randomness

Automatic differentiation (AD), a technique for constructing new programs which compute the derivative of an original program, has become ubiquitous throughout scientific computing and deep learning due to the improved performance afforded by gradient-based optimization. However, AD systems have been restricted to the subset of programs that have a continuous dependence on parameters. Programs that have discrete stochastic behaviors governed by distribution parameters, such as flipping a coin with probability $p$ of being heads, pose a challenge to these systems because the connection between the result (heads vs tails) and the parameters ($p$) is fundamentally discrete. In this paper we develop a new reparameterization-based methodology that allows for generating programs whose expectation is the derivative of the expectation of the original program. We showcase how this method gives an unbiased and low-variance estimator which is as automated as traditional AD mechanisms. We demonstrate unbiased forward-mode AD of discrete-time Markov chains, agent-based models such as Conway's Game of Life, and unbiased reverse-mode AD of a particle filter. Our code package is available at https://github.com/gaurav-arya/StochasticAD.jl.

==> preamble.tex <==
\newcommand{\here}{{\color{red}(\emph{sic})}}
\newcommand{\independent}{\mathop{{\rotatebox[origin=c]{90}{$\models$}}}}
\newcommand{\pder}[2][]{\frac{\dd #1}{\dd #2}}
\makeatletter
\def\lstAZ{A, B, C, D, E, F, G, H, I, J, K, L, M, N, O, P, Q, R, S, T, U, V, W, X, Y, Z}
\def\lstaz{a, b, c, d, e, f, g, h, i, j, k, l, m, n, o, p, q, r, s, t, u, v, w, x, y, z}

\def\lstAZBB{B, C, D, E, F, G, H, I, J, K, L, M, N, O, P, Q, R, T, U, V, W, X, Y, Z}

\newcommand{\MkScr}[1]{\expandafter\def\csname s#1\endcsname{\mathscr{#1}}}
\newcommand{\MkUp}[1]{\expandafter\def\csname u#1\endcsname{\mathrm{#1}}}
\newcommand{\MkFrak}[1]{\expandafter\def\csname f#1\endcsname{\mathfrak{#1}}}
\newcommand{\MkCal}[1]{\expandafter\def\csname c#1\endcsname{\mathcal{#1}}}
\newcommand{\MkBB}[1]{\expandafter\def\csname #1#1\endcsname{\mathbb{#1}}}

\@for\i:=\lstAZ\do{\expandafter\MkScr \i  \expandafter\MkFrak \i  \expandafter\MkUp \i \expandafter\MkCal \i  }    
\@for\i:=\lstaz\do{\expandafter\MkUp \i   }    
	
\@for\i:=\lstAZBB\do{\expandafter\MkBB \i     }
	    
\makeatother

\newcommand{\e}{\mathrm{e}}

\newcommand{\nm}[1]{\mathoperator{#1}}

\newcommand{\ind}{\mathbf{1}}
\newcommand{\id}{\mathbb{1}}

\newcommand{\ds}{\frac{\partial}{\partial s}}
\newcommand{\dt}{\frac{\partial}{\partial t}}
\newcommand{\dr}{\frac{\partial}{\partial r}}

\newcommand{\dd}{ \mathrm{d}}

\DeclareMathOperator{\sgn}{sgn} 
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\renewcommand{\epsilon}{\varepsilon}
 

\newcommand{\vn}[1]{\left| \! \left| #1\right| \! \right|} 
\newcommand{\tn}[1]{\left| \! \left| \! \left|#1\right| \! \right| \! \right|}

\newcommand{\ip}[2]{\langle #1,#2\rangle}


\renewcommand{\tilde}{\widetilde}

\numberwithin{equation}{section}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{theorem2}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{inf_proposition}[theorem]{Informal Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{inf_definition}[theorem]{Informal Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{example}[theorem]{Example}
\newtheorem{condition}[theorem]{Condition}

\DeclareUnicodeCharacter{2202}{$\partial$} \DeclareUnicodeCharacter{2218}{$\circ$} \DeclareUnicodeCharacter{223C}{$\sim$} \DeclareUnicodeCharacter{2207}{$\nabla$} \DeclareUnicodeCharacter{1D53C}{$\mathbb{E}$} 

\newcommand{\xmiddle}[1]{\;\middle#1\;}

